Adaptive Entanglement Generation for Quantum Routing

Entanglement generation in long-distance quantum networks is a difficult process due to resource limitations and the probabilistic nature of entanglement swapping. To maximize success probability, existing quantum routing algorithms employ computationally expensive solutions (e.g., linear programming) to determine which links to entangle and use for end-to-end entanglement generation. Such optimization methods, however, cannot meet the delay requirements of real-world quantum networks, necessitating swift yet efficient real-time optimization models. In this paper, we propose reinforcement learning (RL)-based models to determine which links to entangle and proactively swap to meet connection requests. We show that the proposed RL-based approach is 20x faster compared to linear programming. Moreover, we show that one can take advantage of the longevity of entanglements to (i) cache entangled links for future use and (ii) proactively swap entanglement on high-demand path segments, thereby increasing the likelihood of request success. Through comprehensive simulations, we demonstrate that caching unused entanglements leads to a 10-15% improvement in the performance of state-of-the-art quantum routing algorithms. Complementing caching with proactive entanglement swapping further enhances the request success rate by up to 52.55%.

==> guidelines.tex <==
Articles should not exceed 4500 words through the introduction to conclusion. 
This excludes figures, tables, captions, abstract, and references.


Figures and tables should be limited to a combined total of six (6).


Mathematical equations should not be used. In justified cases, up to three (3) simple equations may be allowed, provided you have the consent of the Guest Editor (GE). The inclusion of more than two equations requires permission from the Editor-in-Chief (EiC).


References should be included only to guide readers to more information on the topic; the reference list should not include every available source. A limit of 15 archival references is recommended. The inclusion of more than 15 references requires permission from the Editor-in-Chief. References to web pages should be checked immediately for accessibility before submitting material to the Publications Staff. Each reference to an online source (website URLs, web-posted articles/reports, etc.) is required to show an “accessed” date.
